Digital Twin of the Radio Environment: A Novel Approach for Anomaly Detection in Wireless Networks

The increasing relevance of resilience in wireless connectivity for Industry 4.0 stems from the growing complexity and interconnectivity of industrial systems, where a single point of failure can disrupt the entire network, leading to significant downtime and productivity losses. It is thus essential to constantly monitor the network and identify any anomaly such as a jammer. Hereby, technologies envisioned to be integrated in 6G, in particular joint communications and sensing (JCAS) and accurate indoor positioning of transmitters, open up the possibility to build a digital twin (DT) of the radio environment. This paper proposes a new approach for anomaly detection in wireless networks enabled by such a DT which allows to integrate contextual information on the network in the anomaly detection procedure. The basic approach is thereby to compare expected received signal strengths (RSSs) from the DT with measurements done by distributed sensing units (SUs). Employing simulations, different algorithms are compared regarding their ability to infer from the comparison on the presence or absence of an anomaly, particular a jammer. Overall, the feasibility of anomaly detection using the proposed approach is demonstrated which integrates in the ongoing research on employing DTs for comprehensive monitoring of wireless networks.

==> results_old.tex <==
\section{Results}
\label{sec:results}

%\enlargethispage{\baselineskip}

The performance of the algorithms under study for anomaly detection as well as the influence of different system model parameters are examined in this section.

To evaluate the performance, a data set is created according to the system model presented in Section~\ref{sec:system_model} containing \num{20000} samples overall. Thereby, \num{10000} normal (i.e., not jammed) samples are used for training and another \num{10000} samples for testing, whereby half of the samples are anomalies and the other half are normal samples. To investigate different shadowing noise levels and densities of \acp{SU}, different data sets are created. Unless otherwise stated in the explanations of the specific algorithms in Section~\ref{sec:unsupervised_learning}, no hyperparameters of the algorithms are tuned, as this would require the evaluation on the test set and thereby mean a leakage of test data (i.e., knowledge of anomalies) into the training phase of the algorithms. After the training phase, the models are evaluated on the test set by means of the metrics presented in the next paragraph. This procedure is repeated three times to improve the reliability of the results. 

The detection is regarded as binary classification problem, where we assign the \textit{positive} class to the anomalies, and the \textit{negative} class are the normal samples. To evaluate the performance of the different algorithms, we first define the two metrics precision and recall 
%
\begin{equation}
    \label{eq:precision_recall}
    \text{precision} = \frac{\mathit{TP}}{\mathit{TP} + \mathit{FP}} \qquad \text{recall} = \frac{\mathit{TP}}{\mathit{TP} + \mathit{FN}}
\end{equation}
%
as in~\cite{chinchor1992muc} with the abbreviations $\mathit{TP}$ for true positive, $\mathit{FP}$ for false positive and $\mathit{FN}$ for false negative. Thus, precision measures how many of the samples classified as anomaly are actually an anomaly, whereas recall measures how many of the anomalies have been correctly identified.

To obtain a comprehensive measure of the performance of anomaly detection, the $F_\beta$ score
%
\begin{equation}
    \label{eq:fbeta_score}
    F_\beta = \frac{(1+\beta^2) \cdot \text{precision} \cdot \text{recall}}{\beta^2 \cdot \text{precision} + \text{recall}}
\end{equation}
%
is employed, which is the weighted harmonic mean of precision and recall~\cite{chinchor1992muc}. As a missed attack is presumably more severe than a false alarm, $\beta = 2$ is employed to weight the recall higher and it is referred to as $F_2$ score in the following. All of the presented metrics range from 0 to 1, whereby 1 denotes an optimal performance.

\begin{figure}
    \centering
    \begin{subfigure}[b]{0.49\columnwidth}
        \centering
        \includegraphics[width=\linewidth]{Figures/both-noise_std.pdf}
        \caption{for different shadowing levels at a measurement grid size of \SI{10}{m}}
        \label{fig:performance-noise}
    \end{subfigure}
    \begin{subfigure}[b]{0.49\columnwidth}
        \centering
        \includegraphics[width=\linewidth]{Figures/both-grid_size.pdf}
        \caption{for different measurement grid sizes at $\sigma=\SI{2}{dB}$}
        \label{fig:performance-grid_size}
    \end{subfigure}
    \caption{Anomaly detection performance}
    \label{fig:performances}
\end{figure}

The performance of the employed methods introduced in Section~\ref{sec:unsupervised_learning} is compared for different scenarios, i.e., different shadowing levels and density of \acp{SU}, in Fig.~\ref{fig:performances}. To improve the performance, the values of \ac{RSS} measurements in each sample are sorted in descending order. This is reasonable, as the location of the jammer currently does not play a role and it reduces the variance in each feature and thus makes it easier to identify samples that significantly differ in the statistics of the \ac{RSS} measurements. While \ac{OCSVM} only slightly benefits, the results of \ac{DBSCAN} improve strongly. The performance of \ac{AED} is not affected as the order does not play a role for averaging.

Considering the $F_2$ score, the different algorithms perform similar in low noise regions as can be seen in Fig.~\ref{fig:performance-noise}. For increasing noise levels, the $F_2$ score of \ac{DBSCAN} and \ac{OCSVM} decreases only slightly (in contrast to \ac{AED}) with \ac{DBSCAN} being constantly the best performing algorithm except for $\sigma=\SI{0}{dB}$. The recall metric is added as second performance metric in the figure, due tot its importance in the given problem mentioned previously. Considering the recall, \ac{DBSCAN} shows by far the best performance, i.e., it correctly identifies most of the actual anomalies.
% However, the $F_1$ score similar to the one of \ac{OCSVM} indicates that this high recall comes at the cost of a high false positive rate, i.e., false alarms. This is a typical trade-off in unsupervised learning.

The grid size of measurements, i.e., the density of \acp{SU} affects the performance similarly as the noise levels. While \ac{AED} has the highest $F_2$ score at the smallest considered grid size of \SI{5}{m}, the other algorithms perform better at larger grid sizes. Some algorithms and scores show better performance with an increasing grid size, e.g., recall and $F_2$ scores of \ac{OCSVM} from \SI{10}{m} to \SI{15}{m}. This might seem counterintuitive but can be explained by the non-optimal parameter selection based only on normal training samples. Further experiments on tuning the parameters of the algorithms manually while taking into account the performance on the test set have shown there are no general optimal parameters for the given problem. Instead, different parameters lead to the best performance in different scenarios (noise level and grid size). The manually tuned parameters also led to strictly descending performances for higher noise levels or larger grid sizes but the results are not shown here, as the tuning based on test results leads to a leakage of knowledge from the test data to the training phase.

Overall, \ac{DBSCAN} shows the best performance in anomaly detection in the examined approach with a recall score greater than 0.8 in all but two examined scenarios, followed by \ac{OCSVM}. The baseline model \ac{AED} suffers from higher noise levels or larger grid sizes of measurements.
